A topology optimisation framework to design test specimens for one-shot identification or discovery of material models

The increasing availability of full-field displacement data from imaging techniques in experimental mechanics is determining a gradual shift in the paradigm of material model calibration and discovery, from using several simple-geometry tests towards a few, or even one single test with complicated geometry. The feasibility of such a "one-shot" calibration or discovery heavily relies upon the richness of the measured displacement data, i.e., their ability to probe the space of the state variables and the stress space (whereby the stresses depend on the constitutive law being sought) to an extent sufficient for an accurate and robust calibration or discovery process. The richness of the displacement data is in turn directly governed by the specimen geometry. In this paper, we propose a density-based topology optimisation framework to optimally design the geometry of the target specimen for calibration of an anisotropic elastic material model. To this end, we perform automatic, high-resolution specimen design by maximising the robustness of the solution of the inverse problem, i.e., the identified material parameters, given noisy displacement measurements from digital image correlation. We discuss the choice of the cost function and the design of the topology optimisation framework, and we analyse a range of optimised topologies generated for the identification of isotropic and anisotropic elastic responses.

==> preamble.tex <==
\usepackage{epsfig}
\usepackage{graphicx}
\usepackage{epstopdf}
\usepackage{subcaption}
\usepackage{floatrow}
\floatsetup[table]{capposition=top}
\usepackage{longtable}
\usepackage{framed}
\usepackage{array,multirow,multicol}
\usepackage{amssymb}
\usepackage{gensymb}
\usepackage[utf8]{inputenc}
\usepackage{dutchcal}
\usepackage{amsthm}
\usepackage{amsmath,bm}
\usepackage{upgreek}
\usepackage{scalerel}
\usepackage{mathtools}
\usepackage{tabularx}
\usepackage{hyperref}
\usepackage[capitalize]{cleveref}
\usepackage{xcolor}
\usepackage{geometry}
\usepackage{makecell}
\usepackage{color, colortbl}
\definecolor{Gray}{gray}{0.8}
\usepackage{enumitem}
\usepackage{outlines}
\usepackage{soul}
\hypersetup{
  colorlinks=true,
  linkcolor=blue
}

\RequirePackage[pagewise]{lineno}

\newcommand{\ten}[1]{\boldsymbol{\mathrm{#1}}}
\newcommand{\smallsquare}{{\scaleto{\square}{3pt}}}
\newcommand{\abs}[1]{\left|#1\right|}
\newcommand{\norm}[1]{\left\|#1\right\|}
\newtheorem{property}{Property}[section]

% Remove the footer for arxiv.org submission
\makeatletter
\def\ps@pprintTitle{\def\@oddfoot{\raggedright\footnotesize Published in \textit{Journal of the Mechanics and Physics of Solids}, 203 (2025) 106210. \url{https://doi.org/10.1016/j.jmps.2025.106210}.}}
\makeatother
